Aspects of Nonrenormalizable Terms in a Superstring Derived Standard--like Model

I investigate the role of nonrenormalizable terms, up to order N=8, in a superstring derived standard--like model. I argue that nonrenormalizable terms restrict the gauge symmetry, at the Planck scale, to be $SU(3)\times SU(2)\times U(1)_{B-L}\times U(1)_{T_{3_R}}$ rather than $SU(3)\times SU(2)\times U(1)_Y$. I show that breaking the gauge symmetry directly to the Standard Model leads to breaking of supersymmetry at the Planck scale, or to dimension four, baryon and lepton violating, operators. I show that if the gauge symmetry is broken directly to the Standard Model the cubic level solution to the F and D flatness constraints is violated by higher order terms, while if $U(1)_{Z^\prime}$ remains unbroken at the Planck scale, the cubic level solution is valid to all orders of nonrenormalizable terms. I discuss the Higgs and fermion mass spectrum. I demonstrate that realistic, hierarchical, fermion mass spectrum can be generated in this model.

==> table1.tex <==
\input tables.tex
\special{landscape}
\hoffset=1.5truein
\nopagenumbers
\magnification=1000
\font\normalroman=cmr10
\font\style=cmr7
\style

\fontdimen12\fivesy=0pt

\textfont0=\sevenrm
\scriptfont0=\fiverm
\textfont1=\seveni
\scriptfont1=\fivei
\textfont2=\sevensy
\scriptfont2=\fivesy

{\hfill
{\begintable
\  \ \|\ $\psi^\mu$ \ \|\ $\{\chi^{12};\chi^{34};\chi^{56}\}$ \ \|\
$y^3y^6$,  $y^4{\bar y}^4$, $y^5{\bar y}^5$,  ${\bar y}^3{\bar y}^6$
\ \|\ $y^1\omega^5$,  $y^2{\bar y}^2$,  $\omega^6{\bar\omega}^6$,
${\bar y}^1{\bar\omega}^5$
\ \|\ $\omega^2{\omega}^4$,  $\omega^1{\bar\omega}^1$,
$\omega^3{\bar\omega}^3$,  ${\bar\omega}^2{\bar\omega}^4$ \ \|\
${\bar\psi}^1$, ${\bar\psi}^2$, ${\bar\psi}^3$,
${\bar\psi}^4$, ${\bar\psi}^5$, ${\bar\eta}^1$,
${\bar\eta}^2$, ${\bar\eta}^3$ \ \|\
${\bar\phi}^1$, ${\bar\phi}^2$, ${\bar\phi}^3$, ${\bar\phi}^4$,
${\bar\phi}^5$, ${\bar\phi}^6$, ${\bar\phi}^7$, ${\bar\phi}^8$ \crthick
$\alpha$
\|\ 0 \|
$\{0,~0,~0\}$ \|
1, ~~~0, ~~~~0, ~~~~0 \|
0, ~~~0, ~~~~1, ~~~~1 \|
0, ~~~0, ~~~~1, ~~~~1 \|
1, ~~1, ~~1, ~~0, ~~0, ~~0 ,~~0, ~~0 \|
1, ~~1, ~~1, ~~1, ~~0, ~~0, ~~0, ~~0 \nr
$\beta$
\|\ 0 \| $\{0,~0,~0\}$ \|
0, ~~~0, ~~~~1, ~~~~1 \|
1, ~~~0, ~~~~0, ~~~~0 \|
0, ~~~1, ~~~~0, ~~~~1 \|
1, ~~1, ~~1, ~~0, ~~0, ~~0, ~~0, ~~0 \|
1, ~~1, ~~1, ~~1, ~~0, ~~0, ~~0, ~~0 \nr
$\gamma$
\|\ 0 \|
$\{0,~0,~0\}$ \|
0, ~~~1, ~~~~0, ~~~~1 \|\
0, ~~~1, ~~~~0, ~~~~1 \|
1, ~~~0, ~~~~0, ~~~~0 \|
{}~~$1\over2$, ~~$1\over2$, ~~$1\over2$, ~~$1\over2$,
{}~~$1\over2$, ~~$1\over2$, ~~$1\over2$, ~~$1\over2$ \| $1\over2$, ~~0, ~~1,
{}~~1,
{}~~$1\over2$,
{}~~$1\over2$, ~~$1\over2$, ~~0 \endtable}
\hfill}
\smallskip
\parindent=0pt
\hangindent=39pt\hangafter=1
\normalroman

{{\it Table 1.} A three generations $SU(3)\times SU(2)\times U(1)^2$ model.
The choice of generalized GSO coeficients is:
$c\left(\matrix{b_j\cr
                                    \alpha,\beta,\gamma\cr}\right)=
-c\left(\matrix{\alpha\cr
                                    1\cr}\right)=
c\left(\matrix{\alpha\cr
                                    \beta\cr}\right)=
-c\left(\matrix{\beta\cr
                                    1\cr}\right)=
c\left(\matrix{\gamma\cr
                                    1,\alpha\cr}\right)=
-c\left(\matrix{\gamma\cr
                                    \beta\cr}\right)=
-1$ (j=1,2,3), with the others specified by modular invariance and space--time
supersymmetry.
Trilevel Yukawa couplings are obtained only for $+{2\over3}$ charged quarks. }
\vskip 2.5cm

\vfill
\eject
\bye


==> table2.tex <==
\input tables.tex
\nopagenumbers
\magnification=1000
\baselineskip=18pt
\hbox
{\hfill
{\begintable
\ F \ \|\ SEC \ \|\ $SU(3)_C$ $\times$ $SU(2)_L$ \ \|\ $Q_C$ & $Q_L$ & $Q_1$ &
$Q_2$
 & $Q_3$ & $Q_4$  & $Q_5$ & $Q_6$
 \ \|\ $SU(5)$ $\times$ $SU(3)$ \ \|\ $Q_7$ &
$Q_8$  \crthick
$V_1$ \|\ ${b_1+2\beta}+(I)$ \|(1,1)\|~0 & ~~0 & ~~0 & ~~${1\over 2}$ &
 ~~$1\over 2$ & ~~$1\over2$
 & ~~0 & ~~0 \|(1,3)\| $-{1\over 2}$ &
{}~~$5\over 2$   \nr
$V_2$ \|\                \|(1,1)\| ~~0 & ~~0 & ~~0 & ~~${1\over 2}$ &
 ~~$1\over 2$ & ~~$1\over2$
  & ~~0 & ~~0
  \|(1,$\bar 3$)\| ~~${1\over 2}$ &
$-{5\over 2}$  \nr
$V_3$ \|\                \|(1,1)\| ~~0 & ~~0 & ~~0 & ~~${1\over 2}$ &
 ~~$1\over 2$ & $-{1\over2}$
  & ~~0 & ~~0
  \|(5,1)\| $-{1\over 2}$ &
$-{3\over 2}$  \nr
$V_4$ \|\                \|(1,1)\| ~~0 & ~~0 & ~~0 & ~~${1\over 2}$ &
 ~~$1\over 2$ & $-{1\over2}$
   & ~~0 & ~~0
  \|($\bar 5$,1)\| ~~$1\over2$ &
{}~~${3\over 2}$  \cr
$V_{5}$ \|\ ${b_2+2\beta}+(I)$ \|(1,1)\| ~~0 & ~~0 &
 ~~${1\over 2}$ & ~~0 &
 ~~$1\over 2$ & ~~0 &  ~~$1\over2$ & ~~0
 \|(1,3)\| $-{1\over 2}$ &
 ~~$5\over 2$  \nr
$V_{6}$ \|\                \|(1,1)\| ~~0 & ~~0 & ~~${1\over 2}$ & ~~0 &
 ~~$1\over 2$ & ~~0 & ~~$1\over2$ & ~~0
  \|(1,$\bar 3$)\| ~~${1\over 2}$ &
 $-{5\over 2}$  \nr
$V_{7}$ \|\                \|(1,1)\| ~~0 & ~~0 & ~~${1\over 2}$ & ~~0 &
 ~~$1\over 2$ & ~~0 & $-{1\over2}$ & ~~0
  \|(5,1)\| $-{1\over 2}$ &
 $-{3\over 2}$ \nr
$V_{8}$ \|\                \|(1,1)\| ~~0 & ~~0 & ~~${1\over 2}$ & ~~0 &
 ~~$1\over 2$ & ~~0 & $-{1\over2}$ & ~~0
  \|($\bar 5$,1)\| ~~$1\over 2$ &
 ~~${3\over 2}$  \cr
$V_{9}$ \|\ ${b_3+2\beta}+(I)$ \|(1,1)\| ~~0 & ~~0 & ~~${1\over 2}$ &
 ~~${1\over 2}$ & ~~0 & ~~0 & ~~0 & ~~${1\over2}$
       \|(1,3)\| $-{1\over 2}$ &
 ~~$5\over 2$  \nr
$V_{10}$ \|\                \|(1,1)\| ~~0 & ~~0 & ~~${1\over 2}$ &
 ~~${1\over 2}$ & ~~0 & ~~0 & ~~0 & ~~$1\over2$
 \|(1,$\bar 3$)\| ~~${1\over 2}$
 & $-{5\over 2}$  \nr
$V_{11}$ \|\                \|(1,1)\| ~~0 & ~~0 & ~~${1\over 2}$ &
 ~~${1\over 2}$ & ~~0 & ~~0 & ~~0 & $-{1\over2}$
       \|(5,1)\|
 $-{1\over 2}$ & $-{3\over 2}$  \nr
$V_{12}$ \|\                \|(1,1)\| ~~0 & ~~0 & ~~${1\over2}$ &
 ~~${1\over 2}$ & ~~0 & ~~0 & ~~0 & $-{1\over2}$
   \|($\bar 5$,1)\| ~~$1\over 2$
 & ~~${3\over 2}$
 \endtable}
\hfill}
\bigskip
\parindent=0pt
\hangindent=39pt\hangafter=1
{\it Table 2.} Massless states
and their quantum numbers. V indicates
that these states form vector representations of the hidden group.

\vfill
\eject
\bye


==> table3.tex <==
\input tables.tex
\nopagenumbers
\magnification=1000
\baselineskip=18pt
\hbox
{\hfill
{\begintable
\ F \ \|\ SEC \ \|\ $SU(3)_C$ $\times$ $SU(2)_L$ \ \|\
$Q_C$ & $Q_L$ & $Q_1$ & $Q_2$ & $Q_3$ & $Q_4$ & $Q_5$ & $Q_6$
  \ \|\ $SU(5)$ $\times$ $SU(3)$ \ \|\ $Q_7$ & $Q_8$  \crthick
$H_1$ \|\
$b_1+b_2+\alpha$ \|(1,1)\|
{}~~${3\over4}$ & ~~${1\over2}$  &  $-{1\over4}$ & $-{1\over4}$ &
{}~~${1\over4}$ &   $-{1\over2}$ &  $-{1\over2}$ & ~~0
 \|(1,3)\|
 ~~${1\over4}$ & $-{5\over4}$   \nr
$H_2$ \|\
$\beta\pm\gamma+(I)$   \|(1,1)\|
  $-{3\over4}$  & $-{1\over2}$  & ~~${1\over4}$ & ~~${1\over4}$ &
  $-{1\over4}$  & $-{1\over2}$  & $-{1\over2}$  & ~~0
\|(1,$\bar 3$)\|
$-{1\over4}$ & ~~${5\over4}$  \nr
$H_3$ \|\
                       \|(1,1)\|
{}~~${3\over4}$   & ~~${1\over2}$  & $-{1\over4}$  &   $-{1\over4}$ &
{}~~${1\over4}$   &   $-{1\over2}$ & $-{1\over2}$  & ~~0
\|(1,1)\|
  $-{3\over4}$  & ~~${{15}\over4}$   \nr
$H_4$ \|\
                       \|(1,1)\|
  $-{3\over4}$  & $-{1\over2}$   & ~~${1\over4}$ & ~~${1\over4}$  &
  $-{1\over4}$  & $-{1\over2}$   & $-{1\over2}$  & ~~0
\|(1,1)\|
{}~~${3\over4}$   & $-{{15}\over4}$    \cr
$H_5$ \|\
$b_1+b_3+\alpha$ \|(1,1)\|
{}~~${3\over4}$   & ~~${1\over2}$  & $-{1\over4}$  & ~~${1\over4}$  &
  $-{1\over4}$  & $-{1\over2}$   & ~~0           &   $-{1\over2}$
\|(1,3)\|
{}~~${1\over4}$   & $-{5\over4}$       \nr
$H_6$ \|\
$\beta\pm\gamma+(I)$  \|(1,1)\|
$-{3\over4}$    & $-{1\over2}$   & ~~${1\over4}$ & $-{1\over4}$   &
{}~~${1\over4}$   & $-{1\over2}$   & ~~0           & $-{1\over2}$
  \|(1,$\bar 3$)\|
  $-{1\over 4}$ & ~~${5\over 4}$     \nr
$H_7$ \|\
               \|(1,1)\|
{}~~${3\over4}$   & ~~${1\over2}$  & $-{1\over4}$  & ~~${1\over4}$  &
  $-{1\over4}$  &   $-{1\over2}$ & ~~0           &   $-{1\over2}$
  \|(1,1)\|
  $-{3\over4}$  &   ${{15}\over4}$   \nr
$H_8$ \|\
                \|(1,1)\|
  $-{3\over4}$  &   $-{1\over2}$ & ~~${1\over4}$ &   $-{1\over4}$ &
  $-{1\over4}$  &   $-{1\over2}$ & ~~0           &   $-{1\over2}$
\|(1,1)\|
{}~~${3\over4}$   & $-{{15}\over4}$    \cr
$H_9$ \|\
$b_2+b_3+\alpha$ \|(1,1)\|
{}~~${3\over4}$   & ~~${1\over2}$  & ~~${1\over4}$ &   $-{1\over4}$ &
  $-{1\over4}$  & ~~0            & $-{1\over2}$  &   $-{1\over2}$
\|(1,3)\|
{}~~${1\over4}$   & $-{5\over4}$       \nr
$H_{10}$ \|\
$\beta\pm\gamma+(I)$  \|(1,1)\|
$-{3\over4}$    & $-{1\over2}$   &  $-{1\over4}$ & ~~${1\over4}$  &
{}~~${1\over4}$   & ~~0            & $-{1\over2}$  &   $-{1\over2}$
  \|(1,$\bar 3$)\|
$-{1\over4}$    & ~~${5\over4}$      \nr
$H_{11}$ \|\
                 \|(1,1)\|
{}~~${3\over4}$   & ~~${1\over2}$  & ~~${1\over4}$ &  $-{1\over4}$  &
  $-{1\over4}$  & ~~0            & $-{1\over2}$  &  $-{1\over2}$
  \|(1,1)\|
  $-{3\over4}$  & ~~${{15}\over4}$   \nr
$H_{12}$ \|\
                \|(1,1)\|
  $-{3\over4}$  &   $-{1\over2}$ &  $-{1\over4}$ & ~~${1\over4}$  &
  $-{1\over4}$  &   ~~0          & $-{1\over2}$  &  $-{1\over2}$
\|(1,1)\|
{}~~${3\over4}$   & $-{{15}\over4}$    \cr
$H_{13}$ \|\
$b_1+b_3+\alpha$ \|(1,1)\|
 $-{3\over4}$   & ~~${1\over2}$  &  $-{1\over4}$ &  ~~${1\over4}$ &
  $-{1\over4}$  & ~~0            & ~~0           &   ~~0
\|(1,3)\|
{}~~${3\over4}$   & ~~${5\over4}$       \nr
$H_{14}$ \|\
$\pm\gamma+(I)$  \|(1,1)\|
{}~~${3\over4}$   & $-{1\over2}$   & ~~${1\over4}$ &  $-{1\over4}$  &
{}~~${1\over4}$   & ~~0            & ~~0           & ~~0
  \|(1,$\bar 3$)\|
$-{3\over4}$    &  $-{5\over4}$      \nr
$H_{15}$ \|\
                 \|(1,2)\|
 $-{3\over4}$   &  $-{1\over2}$  &  $-{1\over4}$ & ~~${1\over4}$  &
  $-{1\over4}$  & ~~0            & ~~0           &  ~~0
  \|(1,1)\|
  $-{1\over4}$  &   $-{{15}\over4}$   \nr
$H_{16}$ \|\
                \|(1,2)\|
 ~~${3\over4}$  & ~~${1\over2}$  & ~~${1\over4}$ &  $-{1\over4}$  &
 ~~${1\over4}$  &   ~~0          & ~~0           &  ~~0
\|(1,1)\|
{}~~${1\over4}$   & ~~${{15}\over4}$    \nr
$H_{17}$ \|\
                 \|(1,1)\|
 $-{3\over4}$   & ~~${1\over2}$  &  $-{1\over4}$ &  $-{3\over4}$  &
 $-{1\over4}$   & ~~0            & ~~0           & ~~0
  \|(1,1)\|
$-{1\over4}$    &  $-{{15}\over4}$    \nr
$H_{18}$ \|\
                 \|(1,1)\|
 ~~${3\over4}$  &  $-{1\over2}$  & ~~${1\over4}$ & ~~${3\over4}$  &
 ~~${1\over4}$  & ~~0            & ~~0           &  ~~0
  \|(1,1)\|
 ~~${1\over4}$  &  ~~${{15}\over4}$   \cr
$H_{19}$ \|\
$b_2+b_3+\alpha$ \|(1,1)\|
 $-{3\over4}$   & ~~${1\over2}$  & ~~${1\over4}$ &   $-{1\over4}$ &
  $-{1\over4}$  & ~~0            & ~~0           &   ~~0
\|(5,1)\|
 $-{1\over4}$   & ~~${9\over4}$       \nr
$H_{20}$ \|\
$\pm\gamma+(I)$  \|(1,1)\|
{}~~${3\over4}$   & $-{1\over2}$   &  $-{1\over4}$ & ~~${1\over4}$  &
{}~~${1\over4}$   & ~~0            & ~~0           & ~~0
  \|($\bar 5$,1)\|
{}~~${1\over4}$   &  $-{9\over4}$      \nr
$H_{21}$ \|\
                 \|(3,1)\|
{}~~${3\over4}$   & ~~${1\over2}$  & ~~${1\over4}$ &  $-{1\over4}$  &
  $-{1\over4}$  & ~~0            & ~~0           &  ~~0
  \|(1,1)\|
  $-{1\over4}$  &   $-{{15}\over4}$   \nr
$H_{22}$ \|\
                \|($\bar 3$,1)\|
  $-{1\over4}$  &  $-{1\over2}$  &  $-{1\over4}$ & ~~${1\over4}$  &
 ~~${1\over4}$  &   ~~0          & ~~0           &  ~~0
\|(1,1)\|
{}~~${1\over4}$   & ~~${{15}\over4}$    \nr
$H_{23}$ \|\
                 \|(1,1)\|
 $-{3\over4}$   & ~~${1\over2}$  & ~~${1\over4}$ &  $-{1\over4}$  &
{}~~${1\over4}$   & ~~0            & ~~0           & ~~0
  \|(1,1)\|
$-{1\over4}$    &  $-{{15}\over4}$    \nr
$H_{24}$ \|\
                 \|(1,1)\|
 ~~${3\over4}$  &  $-{1\over2}$  &  $-{1\over4}$ & ~~${1\over4}$  &
  $-{3\over4}$  & ~~0            & ~~0           &  ~~0
  \|(1,1)\|
 ~~${1\over4}$  &  ~~${{15}\over4}$   \nr
$H_{25}$ \|\
                \|(1,1)\|
  $-{3\over4}$  & ~~${1\over2}$  & ~~${1\over4}$ &  ~~${3\over4}$ &
  $-{1\over4}$  &   ~~0          & ~~0           &  ~~0
\|(1,1)\|
 $-{1\over4}$   &  $-{{15}\over4}$    \nr
$H_{26}$ \|\
                \|(1,1)\|
 ~~${3\over4}$  &  $-{1\over2}$  &  $-{1\over4}$ &   $-{3\over4}$ &
 ~~${1\over4}$  &   ~~0          & ~~0           &  ~~0
\|(1,1)\|
 ~~${1\over4}$  &  ~~${{15}\over4}$    \cr
$H_{27}$ \|\
                 \|(1,1)\|
 $-{3\over4}$   &  $-{1\over2}$  &  $-{1\over4}$ &  $-{1\over4}$  &
 $-{1\over4}$   &  $-{1\over2}$  & ~~${1\over2}$ & ~~${1\over2}$
  \|(1,1)\|
{}~~${1\over4}$    &  $-{{5}\over4}$    \nr
$H_{28}$ \|\
                 \|(1,1)\|
 ~~${3\over4}$  & ~~${1\over2}$  & ~~${1\over4}$ & ~~${1\over4}$  &
 ~~${1\over4}$  & ~~${1\over2}$  & $-{1\over2}$  &  $-{1\over2}$
  \|(1,1)\|
 $-{1\over4}$  &  ~~${{5}\over4}$   \nr
$H_{29}$ \|\
                \|(1,1)\|
  $-{3\over4}$  & $-{1\over2}$  &  $-{1\over4}$ &   $-{1\over4}$ &
  $-{1\over4}$  & ~~${1\over2}$  & $-{1\over2}$ &  ~~${1\over2}$
\|(1,1)\|
 $-{3\over4}$   &  ~~${{15}\over4}$    \nr
$H_{30}$ \|\
                \|(1,1)\|
 ~~${3\over4}$  & ~~${1\over2}$  & ~~${1\over4}$ &  ~~${1\over4}$ &
 ~~${1\over4}$  &  $-{1\over2}$  & ~~${1\over2}$ &  $-{1\over2}$
\|(1,1)\|
 ~~${3\over4}$  &  $-{{15}\over4}$
\endtable}
\hfill}
\bigskip
\parindent=0pt
\hangindent=39pt\hangafter=1
{\it Table 3.} Massless states and their quantum numbers.



\end
\bye

